Ultra-Reliable Device-Centric Uplink Communications in Airborne Networks: A Spatiotemporal Analysis

This paper proposes an ultra-reliable device-centric uplink (URDC-UL) communication scheme for airborne networks. In particular, base stations (BSs) are mounted on unmanned aerial vehicles (UAVs) that travel to schedule UL transmissions and collect data from devices. To attain an ultra-reliable unified device-centric performance, the UL connection is established when the UAV-BS is hovering at the nearest possible distance from the scheduled device. The performance of the proposed URDC-UL scheme is benchmarked against a stationary UAV-centric uplink (SUC-UL) scheme where the devices are scheduled to communicate to UAV-BSs that are continuously hovering at static locations. Utilizing stochastic geometry and queueing theory, novel spatiotemporal mathematical models are developed, which account for the UAV-BS spatial densities, mobility, altitude, antenna directivity, ground-to-air channel, and temporal traffic, among other factors. The results demonstrate the sensitivity of the URDC-UL scheme to the ratio between hovering and traveling time. In particular, the hovering to traveling time ratio should be carefully adjusted to maximize the harvested performance gains for the URDC-UL scheme in terms of link reliability, transmission rate, energy efficiency, and delay. Exploiting the URDC-UL scheme allows IoT devices to minimize transmission power while maintaining unified reliable transmission. This preserves the device's battery and addresses a critical IoT design challenge.

==> P_LOS_sd.tex <==
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{axis}[%
width=3in,
height=2.3in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={$\eta$},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{P}_{\text{LOS}}$},
axis background/.style={fill=white},
legend style={font=\footnotesize,at={(0.01,0.01)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
grid=both
]
\addplot [line width=0.6mm,color=mycolor1]
  table[row sep=crcr]{%
1	1.00000000000004\\
2	1.00000000000001\\
3	1.00000000001186\\
4	1.00000000224915\\
5	1.00000000000135\\
6	0.999999999995351\\
7	0.999999999954688\\
8	1.00000000157115\\
9	0.999999999087998\\
10	0.999999996776252\\
11	0.999999990007098\\
12	0.99999997249339\\
13	0.999999931604997\\
14	0.999999843316568\\
15	0.999999667851677\\
16	0.999999342142001\\
17	0.999998763450844\\
18	0.999997795287653\\
19	0.999996240056295\\
20	0.999993835858232\\
21	0.999990243706137\\
22	0.999985037100582\\
23	0.999977692843036\\
24	0.999967583482296\\
25	0.999953971671113\\
26	0.999936006676416\\
27	0.999912723293007\\
28	0.999883043447565\\
29	0.99984578026962\\
30	0.999799642917379\\
31	0.999743245365026\\
32	0.99967511592212\\
33	0.999593708450581\\
34	0.999497414758608\\
35	0.99938457785137\\
36	0.999253505721463\\
37	0.999102485375531\\
38	0.998929796815244\\
39	0.998733726718765\\
40	0.998512581601\\
41	0.99826470026551\\
42	0.997988465396254\\
43	0.997682314172031\\
44	0.997344747819444\\
45	0.996974340050679\\
46	0.996569744359799\\
47	0.996129700175446\\
48	0.99565303788861\\
49	0.995138682791528\\
50	0.994585657977951\\
51	0.993993086265972\\
52	0.99336019121269\\
53	0.992686297295372\\
54	0.991970829336774\\
55	0.991213311253364\\
56	0.990413364204551\\
57	0.989570704219207\\
58	0.988685139372916\\
59	0.987756566585887\\
60	0.986784968298676\\
61	0.985770407994652\\
62	0.984713027189573\\
63	0.983613040774101\\
64	0.982470732937929\\
65	0.981286452919296\\
66	0.980060610738665\\
67	0.978793672949432\\
68	0.977486158434237\\
69	0.976138635067394\\
70	0.974751712636181\\
71	0.973326043151537\\
72	0.971862313504963\\
73	0.970361246349446\\
74	0.968823590478154\\
75	0.967250121503265\\
76	0.965641637628027\\
77	0.963998956577644\\
78	0.962322912689582\\
79	0.960614354163315\\
80	0.958874140468426\\
81	0.957103139908928\\
82	0.955302227340897\\
83	0.953472282039764\\
84	0.951614185713109\\
85	0.949728820654287\\
86	0.947817068031907\\
87	0.945879806309919\\
88	0.943917909792841\\
89	0.941932247290601\\
90	0.939923686388161\\
91	0.937893064878565\\
92	0.93584124466106\\
93	0.93376905591999\\
94	0.931677323757808\\
95	0.929566861969618\\
96	0.927438472389854\\
97	0.925292944315245\\
98	0.923131053999236\\
99	0.920953564213211\\
100	0.918761223870032\\
};
\addlegendentry{\normalsize{Suburban}}

\addplot [line width=0.6mm,color=mycolor2]
  table[row sep=crcr]{%
1	0.999962087456531\\
2	0.999949054994084\\
3	0.999928777950083\\
4	0.999896588303821\\
5	0.999845082480279\\
6	0.999763148255037\\
7	0.999635045655223\\
8	0.999439869851605\\
9	0.999151552227205\\
10	0.998739554977465\\
11	0.998170155848552\\
12	0.997408200954671\\
13	0.996419033462883\\
14	0.995170344551104\\
15	0.993633737559703\\
16	0.991785873794213\\
17	0.989609162838954\\
18	0.987092011613457\\
19	0.984228726496374\\
20	0.981019113191893\\
21	0.977467906712885\\
22	0.973584086143012\\
23	0.969380148362978\\
24	0.964871388933921\\
25	0.960075224384322\\
26	0.955010577293263\\
27	0.949697335443281\\
28	0.94415588882223\\
29	0.938406743030998\\
30	0.93247020427955\\
31	0.926366129213063\\
32	0.92011373192122\\
33	0.913731440314317\\
34	0.907236794332954\\
35	0.90064637900153\\
36	0.893975785599641\\
37	0.887239598270059\\
38	0.880451393240988\\
39	0.87362375773256\\
40	0.866768316799464\\
41	0.859895768517637\\
42	0.853015924676183\\
43	0.846137755095504\\
44	0.839269436236835\\
45	0.832418387735752\\
46	0.825591341475146\\
47	0.818794366591097\\
48	0.812032925782266\\
49	0.805311916998515\\
50	0.798635715420545\\
51	0.792008213386632\\
52	0.785432858164406\\
53	0.778912687522867\\
54	0.772450363103878\\
55	0.766048201625752\\
56	0.759708203976336\\
57	0.753432082270806\\
58	0.74722128496177\\
59	0.741077020097256\\
60	0.735000276826774\\
61	0.728991845257609\\
62	0.723052334763394\\
63	0.717182190845403\\
64	0.711381710644229\\
65	0.705651057195909\\
66	0.699990272522362\\
67	0.694399289641522\\
68	0.688877943577736\\
69	0.683425981448262\\
70	0.678043071696876\\
71	0.672728812540935\\
72	0.66748273959742\\
73	0.662304333438941\\
74	0.657193025140916\\
75	0.652148202819886\\
76	0.647169216816499\\
77	0.642255384578972\\
78	0.637405995110075\\
79	0.632620313013739\\
80	0.627897582174519\\
81	0.623237029100511\\
82	0.618637865957883\\
83	0.614099292865684\\
84	0.609620502554083\\
85	0.605200678950947\\
86	0.600839001877987\\
87	0.596534646891463\\
88	0.592286791609895\\
89	0.588094611030756\\
90	0.583957282466464\\
91	0.579873985969932\\
92	0.575843905411444\\
93	0.571866229439824\\
94	0.567940152337956\\
95	0.564064874781857\\
96	0.560239604511782\\
97	0.556463556923083\\
98	0.552735955583939\\
99	0.549056032686444\\
100	0.545423029437028\\
};
\addlegendentry{\normalsize{Urban}}

\addplot [line width=0.6mm,color=mycolor3]
  table[row sep=crcr]{%
1	0.997992022385056\\
2	0.997546867617451\\
3	0.996948525022649\\
4	0.996141309737144\\
5	0.995056231784931\\
6	0.993613691361334\\
7	0.991729106669462\\
8	0.989320631014011\\
9	0.986317144902978\\
10	0.982664722446074\\
11	0.978330441347273\\
12	0.973303323875566\\
13	0.9675928959253\\
14	0.96122617004381\\
15	0.954243863153539\\
16	0.946696489284481\\
17	0.938640751010132\\
18	0.930136453315274\\
19	0.921244033949324\\
20	0.912022677913325\\
21	0.902528973846677\\
22	0.892816014287447\\
23	0.882932854836661\\
24	0.872924248946334\\
25	0.862830586893542\\
26	0.852687980129035\\
27	0.842528444320904\\
28	0.832380145134699\\
29	0.822267679777008\\
30	0.812212374595312\\
31	0.802232584751119\\
32	0.792343986396455\\
33	0.782559855113862\\
34	0.772891326835628\\
35	0.763347639225875\\
36	0.753936352564985\\
37	0.74466355164279\\
38	0.735534025129824\\
39	0.726551429563655\\
40	0.717718434510047\\
41	0.709036852120493\\
42	0.700507752163237\\
43	0.692131564494477\\
44	0.683908165993046\\
45	0.675836966002848\\
46	0.667916970040234\\
47	0.660146844177822\\
48	0.652524968224757\\
49	0.645049482831965\\
50	0.637718330679706\\
51	0.630529292435363\\
52	0.623480018095547\\
53	0.616568054259178\\
54	0.609790867817036\\
55	0.603145866488119\\
56	0.596630416583711\\
57	0.590241858335822\\
58	0.583975789402109\\
59	0.577834724606148\\
60	0.571810808754744\\
61	0.565903121718906\\
62	0.560109036975313\\
63	0.554425957156082\\
64	0.548851318949448\\
65	0.543382597159042\\
66	0.538017308029428\\
67	0.532753011932553\\
68	0.527587315498275\\
69	0.522517873262012\\
70	0.517542388893647\\
71	0.512658616064015\\
72	0.507864358954731\\
73	0.503157472810781\\
74	0.498535863469669\\
75	0.493997487622285\\
76	0.489540352387074\\
77	0.485162514853266\\
78	0.480862081503927\\
79	0.476637207538517\\
80	0.472486096112184\\
81	0.46840699750682\\
82	0.464398207781999\\
83	0.460458069918989\\
84	0.456584969502089\\
85	0.452777336081153\\
86	0.449033640814817\\
87	0.445352398041707\\
88	0.44173216099\\
89	0.438171522556862\\
90	0.434669113923817\\
91	0.431223603544523\\
92	0.427833696142203\\
93	0.424498131719217\\
94	0.421215684580875\\
95	0.417985162375202\\
96	0.414805405150076\\
97	0.411675284428875\\
98	0.408593702305544\\
99	0.405559590559771\\
100	0.40257190979279\\
};
\addlegendentry{\normalsize{Dense Urban}}

\addplot [line width=0.6mm,color=mycolor4]
  table[row sep=crcr]{%
1	0.813125188658297\\
2	0.793383232426189\\
3	0.771860935354024\\
4	0.748945195127941\\
5	0.725113466208481\\
6	0.700851063584671\\
7	0.676589866626187\\
8	0.652678285555345\\
9	0.629375873905767\\
10	0.606861941202572\\
11	0.585249793378344\\
12	0.564601659691743\\
13	0.544941978747503\\
14	0.526268266085732\\
15	0.50855956200344\\
16	0.491782778352616\\
17	0.475897348210649\\
18	0.460858562256659\\
19	0.446619916827609\\
20	0.433134731139461\\
21	0.420357232034715\\
22	0.408243256945676\\
23	0.396750681050732\\
24	0.385839659346666\\
25	0.375472726390907\\
26	0.365614811822816\\
27	0.35623319251898\\
28	0.347297406158807\\
29	0.338779139176434\\
30	0.330652112829458\\
31	0.322891935746241\\
32	0.315475993095734\\
33	0.308383310649563\\
34	0.301594434948682\\
35	0.295091317860262\\
36	0.288857208089256\\
37	0.282876549934152\\
38	0.277134889294871\\
39	0.271618786755342\\
40	0.266315737446254\\
41	0.261214097324037\\
42	0.256303015465403\\
43	0.251572371961975\\
44	0.247012720999488\\
45	0.242615238160353\\
46	0.238371674782811\\
47	0.234274311358977\\
48	0.230315919141041\\
49	0.226489723063705\\
50	0.222789368097689\\
51	0.219208888398591\\
52	0.21574267900445\\
53	0.212385469856673\\
54	0.209132301938901\\
55	0.205978505346766\\
56	0.202919677135376\\
57	0.199951672671383\\
58	0.197070568704922\\
59	0.194272667441108\\
60	0.1915544720882\\
61	0.188912675421644\\
62	0.186344147387179\\
63	0.183845923639409\\
64	0.181415194937136\\
65	0.179049297323884\\
66	0.176745703028565\\
67	0.174502012027064\\
68	0.172315944210838\\
69	0.170185332113439\\
70	0.168108114150172\\
71	0.166082328330078\\
72	0.164106106402975\\
73	0.162177668407528\\
74	0.160295317589246\\
75	0.15845743566\\
76	0.156662478373027\\
77	0.154908971389626\\
78	0.153195506415719\\
79	0.151520737588287\\
80	0.14988337809333\\
81	0.148282196998491\\
82	0.146716016284873\\
83	0.145183708063815\\
84	0.143684191965494\\
85	0.142216432687305\\
86	0.140779437690878\\
87	0.139372254801113\\
88	0.13799397104203\\
89	0.136643709531296\\
90	0.135320628392364\\
91	0.134023918894144\\
92	0.132752803849175\\
93	0.131506536102969\\
94	0.130284397108575\\
95	0.129085695580871\\
96	0.127909766225476\\
97	0.126755968537541\\
98	0.125623685666018\\
99	0.124512323339314\\
100	0.123421308848537\\
};
\addlegendentry{\normalsize{High-rise Urban}}

\end{axis}


==> approx1_sim.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{axis}[%
width=3in,
height=2.3in,
at={(0.758in,0.481in)},
scale only axis,
xmin=-20,
xmax=65,
xtick={-20,-10,...,80},
xlabel style={font=\large \color{white!15!black}},
xlabel={SINR Threshold (dB)},
ymin=0,
ymax=1,
ticklabel style={font=\normalsize},
ylabel style={font=\large \color{white!15!black}},
ylabel={Success probability},
axis background/.style={fill=white},
legend style={font=\footnotesize,at={(0.22,0.42)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
  grid=both,
]
\addplot [line width=0.6mm,color=mycolor1, dashdotted]
  table[row sep=crcr]{%
-20	1\\
-19	1\\
-18	1\\
-17	1\\
-16	1\\
-15	1\\
-14	1\\
-13	1\\
-12	1\\
-11	1\\
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	0.9995\\
13	0.9995\\
14	0.9995\\
15	0.9995\\
16	0.9995\\
17	0.9995\\
18	0.999\\
19	0.999\\
20	0.999\\
21	0.9985\\
22	0.9985\\
23	0.9975\\
24	0.9975\\
25	0.9975\\
26	0.996\\
27	0.995\\
28	0.9925\\
29	0.9915\\
30	0.99\\
31	0.9895\\
32	0.988\\
33	0.986\\
34	0.982\\
35	0.9775\\
36	0.975\\
37	0.97\\
38	0.9635\\
39	0.9565\\
40	0.951\\
41	0.946\\
42	0.9355\\
43	0.919\\
44	0.9015\\
45	0.885\\
46	0.863\\
47	0.8345\\
48	0.801\\
49	0.7595\\
50	0.7055\\
51	0.635\\
52	0.557\\
53	0.494\\
54	0.413\\
55	0.319\\
56	0.2445\\
57	0.1685\\
58	0.1055\\
59	0.059\\
60	0.036\\
61	0.015\\
62	0.005\\
63	0.0025\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
71	0\\
72	0\\
73	0\\
74	0\\
75	0\\
76	0\\
77	0\\
78	0\\
79	0\\
80	0\\
};
\addlegendentry{URDC-UL exact}

\addplot [line width=0.6mm,color=mycolor2, dashdotted]
  table[row sep=crcr]{%
-20	1\\
-19	1\\
-18	1\\
-17	1\\
-16	1\\
-15	1\\
-14	1\\
-13	1\\
-12	1\\
-11	1\\
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	0.9995\\
15	0.9995\\
16	0.9995\\
17	0.9995\\
18	0.9995\\
19	0.9995\\
20	0.999\\
21	0.9985\\
22	0.998\\
23	0.997\\
24	0.997\\
25	0.997\\
26	0.996\\
27	0.995\\
28	0.995\\
29	0.9935\\
30	0.9935\\
31	0.9915\\
32	0.9905\\
33	0.989\\
34	0.987\\
35	0.9845\\
36	0.982\\
37	0.98\\
38	0.973\\
39	0.967\\
40	0.964\\
41	0.9555\\
42	0.9415\\
43	0.93\\
44	0.915\\
45	0.896\\
46	0.874\\
47	0.846\\
48	0.813\\
49	0.7715\\
50	0.7255\\
51	0.6615\\
52	0.595\\
53	0.526\\
54	0.442\\
55	0.3495\\
56	0.2575\\
57	0.192\\
58	0.1265\\
59	0.072\\
60	0.0395\\
61	0.0145\\
62	0.006\\
63	0.002\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
71	0\\
72	0\\
73	0\\
74	0\\
75	0\\
76	0\\
77	0\\
78	0\\
79	0\\
80	0\\
};
\addlegendentry{URDC-UL PPP}


\addplot [line width=0.6mm,color=mycolor3, dashdotted]
  table[row sep=crcr]{%
-20	0.6785\\
-19	0.644\\
-18	0.5995\\
-17	0.5585\\
-16	0.5165\\
-15	0.4805\\
-14	0.4475\\
-13	0.417\\
-12	0.389\\
-11	0.363\\
-10	0.3425\\
-9	0.321\\
-8	0.3055\\
-7	0.2855\\
-6	0.2745\\
-5	0.2645\\
-4	0.2565\\
-3	0.249\\
-2	0.244\\
-1	0.2395\\
0	0.2365\\
1	0.2325\\
2	0.231\\
3	0.2275\\
4	0.2265\\
5	0.225\\
6	0.224\\
7	0.2215\\
8	0.2185\\
9	0.217\\
10	0.217\\
11	0.2155\\
12	0.2145\\
13	0.2135\\
14	0.2125\\
15	0.2115\\
16	0.2085\\
17	0.2045\\
18	0.2\\
19	0.1955\\
20	0.1905\\
21	0.1855\\
22	0.1775\\
23	0.1695\\
24	0.1625\\
25	0.1495\\
26	0.1405\\
27	0.1275\\
28	0.1185\\
29	0.1095\\
30	0.1005\\
31	0.0895\\
32	0.08\\
33	0.0725\\
34	0.0645\\
35	0.0555\\
36	0.045\\
37	0.039\\
38	0.0305\\
39	0.026\\
40	0.0225\\
41	0.0185\\
42	0.0155\\
43	0.013\\
44	0.011\\
45	0.008\\
46	0.007\\
47	0.005\\
48	0.0035\\
49	0.0035\\
50	0.003\\
51	0.0025\\
52	0.0015\\
53	0.0005\\
54	0.0005\\
55	0.0005\\
56	0\\
57	0\\
58	0\\
59	0\\
60	0\\
61	0\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
71	0\\
72	0\\
73	0\\
74	0\\
75	0\\
76	0\\
77	0\\
78	0\\
79	0\\
80	0\\
};
\addlegendentry{SUC-UL  exact}

\addplot [line width=0.6mm,color=mycolor4, dashdotted]
  table[row sep=crcr]{%
-20	0.6585\\
-19	0.6185\\
-18	0.5865\\
-17	0.5455\\
-16	0.5115\\
-15	0.4825\\
-14	0.453\\
-13	0.4255\\
-12	0.3995\\
-11	0.3745\\
-10	0.3505\\
-9	0.3285\\
-8	0.309\\
-7	0.2905\\
-6	0.279\\
-5	0.267\\
-4	0.2545\\
-3	0.2445\\
-2	0.2375\\
-1	0.233\\
0	0.228\\
1	0.2245\\
2	0.2235\\
3	0.223\\
4	0.221\\
5	0.2205\\
6	0.2175\\
7	0.216\\
8	0.2155\\
9	0.2145\\
10	0.2135\\
11	0.211\\
12	0.2105\\
13	0.2075\\
14	0.2045\\
15	0.202\\
16	0.2005\\
17	0.197\\
18	0.1925\\
19	0.187\\
20	0.1835\\
21	0.1745\\
22	0.1675\\
23	0.162\\
24	0.152\\
25	0.143\\
26	0.135\\
27	0.1285\\
28	0.118\\
29	0.106\\
30	0.098\\
31	0.085\\
32	0.075\\
33	0.068\\
34	0.061\\
35	0.052\\
36	0.0415\\
37	0.0345\\
38	0.031\\
39	0.027\\
40	0.025\\
41	0.021\\
42	0.017\\
43	0.0135\\
44	0.0105\\
45	0.008\\
46	0.006\\
47	0.0035\\
48	0.0025\\
49	0.0015\\
50	0.0005\\
51	0\\
52	0\\
53	0\\
54	0\\
55	0\\
56	0\\
57	0\\
58	0\\
59	0\\
60	0\\
61	0\\
62	0\\
63	0\\
64	0\\
65	0\\
66	0\\
67	0\\
68	0\\
69	0\\
70	0\\
71	0\\
72	0\\
73	0\\
74	0\\
75	0\\
76	0\\
77	0\\
78	0\\
79	0\\
80	0\\
};
\addlegendentry{SUC-UL  PPP}

\end{axis}


==> environment2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%


\begin{axis}[%
width=3in,
height=2.3in,
at={(0.1158in,0.081in)},
scale only axis,
xmin=-10,
xmax=35,
xlabel style={font=\color{white!15!black}},
xlabel={SIR Threshold (db)},
ymin=0.65,
ymax=1.05,
ylabel style={font=\color{white!15!black}},
ylabel={Success probability},
axis background/.style={fill=white},
legend style={font=\footnotesize,at={(0.03,0.06)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
-10	0.999999999990627\\
-9	0.999999999981316\\
-8	0.999999999962731\\
-7	0.999999999925702\\
-6	0.999999999851895\\
-5	0.999999999704858\\
-4	0.99999999941201\\
-3	0.999999998829075\\
-2	0.999999997669361\\
-1	0.999999995363903\\
0	0.999999990785127\\
1	0.999999981702069\\
2	0.999999963710283\\
3	0.999999928137599\\
4	0.999999857965775\\
5	0.999999719936598\\
6	0.99999944938788\\
7	0.999998921394436\\
8	0.999997896473621\\
9	0.99999591986075\\
10	0.999992137798893\\
11	0.999984969222935\\
12	0.999971532940164\\
13	0.99994667564314\\
14	0.99990137368018\\
15	0.999820194415698\\
16	0.999677409887156\\
17	0.99943127283081\\
18	0.999015926882307\\
19	0.998330507917793\\
20	0.997225365013986\\
21	0.995486215482964\\
22	0.992818549742674\\
23	0.988836345711692\\
24	0.983060192841967\\
25	0.974929427619314\\
26	0.963831240884207\\
27	0.949148372644772\\
28	0.930325914464174\\
29	0.906953380239682\\
30	0.8788471548474\\
31	0.846105018400821\\
32	0.809101903981475\\
33	0.768414450209753\\
34	0.724694263107389\\
35	0.678534812025225\\
36	0.630378048252149\\
37	0.580486638528962\\
38	0.52898239498624\\
39	0.475935212217175\\
40	0.421482320937835\\
};
\addlegendentry{Suburnan}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
-10	0.999999999998481\\
-9	0.999999999996979\\
-8	0.999999999993964\\
-7	0.999999999987971\\
-6	0.999999999976017\\
-5	0.999999999952212\\
-4	0.999999999904787\\
-3	0.999999999810394\\
-2	0.999999999622594\\
-1	0.999999999249221\\
0	0.999999998507652\\
1	0.999999997036449\\
2	0.999999994121963\\
3	0.999999988358785\\
4	0.999999976988249\\
5	0.999999954617471\\
6	0.999999910757242\\
7	0.999999825132578\\
8	0.999999658851479\\
9	0.999999338000463\\
10	0.999998723674297\\
11	0.999997558294948\\
12	0.99999537167049\\
13	0.999991320928058\\
14	0.999983925769357\\
15	0.999970644359647\\
16	0.999947215818135\\
17	0.999906673142933\\
18	0.999837906906496\\
19	0.999723641894206\\
20	0.99953769593226\\
21	0.999241458102715\\
22	0.998779681298293\\
23	0.998075902222096\\
24	0.997027966736869\\
25	0.995504145385149\\
26	0.993340269232103\\
27	0.990338513699097\\
28	0.98626900086507\\
29	0.980875572741092\\
30	0.97388565704862\\
31	0.965020795416249\\
32	0.954001074300367\\
33	0.94053658003235\\
34	0.924303463536518\\
35	0.904908995689877\\
36	0.881855170867907\\
37	0.854512041595065\\
38	0.822111543450695\\
39	0.783772994847759\\
40	0.738574014203753\\
};
\addlegendentry{Urban}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
-10	0.999999999998975\\
-9	0.999999999997966\\
-8	0.999999999995931\\
-7	0.999999999991894\\
-6	0.999999999983836\\
-5	0.999999999967793\\
-4	0.999999999935829\\
-3	0.999999999872211\\
-2	0.999999999745636\\
-1	0.999999999493974\\
0	0.999999998994127\\
1	0.999999998002431\\
2	0.999999996037741\\
3	0.999999992152429\\
4	0.999999984486147\\
5	0.999999969401496\\
6	0.999999939822215\\
7	0.999999882066689\\
8	0.999999769881785\\
9	0.999999553353357\\
10	0.999999138630015\\
11	0.99999835156899\\
12	0.999996874036856\\
13	0.999994135201003\\
14	0.999989131377515\\
15	0.999980136731776\\
16	0.999964253417662\\
17	0.999936733693614\\
18	0.99988998881476\\
19	0.999812184014145\\
20	0.99968531822348\\
21	0.99948272462956\\
22	0.999166023553779\\
23	0.998681694947796\\
24	0.997957540573683\\
25	0.996899306082362\\
26	0.995387693239826\\
27	0.993276126773859\\
28	0.990390031393405\\
29	0.986528572384179\\
30	0.981468955435358\\
31	0.974971156402619\\
32	0.966778533590504\\
33	0.956609297062381\\
34	0.944136388538778\\
35	0.928957729735439\\
36	0.910562528426399\\
37	0.88830107145056\\
38	0.861366171439011\\
39	0.828796296017141\\
40	0.789514627766903\\
};
\addlegendentry{Dense Urban}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
-10	0.999999999999834\\
-9	0.999999999999677\\
-8	0.999999999999343\\
-7	0.999999999998696\\
-6	0.999999999997395\\
-5	0.999999999994816\\
-4	0.999999999989664\\
-3	0.999999999979425\\
-2	0.99999999995905\\
-1	0.999999999918526\\
0	0.999999999838059\\
1	0.999999999678413\\
2	0.999999999362139\\
3	0.999999998736719\\
4	0.999999997502755\\
5	0.999999995074906\\
6	0.999999990314646\\
7	0.99999998102108\\
8	0.999999962972007\\
9	0.999999928142357\\
10	0.999999861448919\\
11	0.999999734918616\\
12	0.999999497481635\\
13	0.999999057577607\\
14	0.999998254383915\\
15	0.999996811720036\\
16	0.999994266567581\\
17	0.999989861687627\\
18	0.999982389077533\\
19	0.99996996852444\\
20	0.999949745139427\\
21	0.999917495078934\\
22	0.99986714281934\\
23	0.999790213586228\\
24	0.999675258899192\\
25	0.999507289811807\\
26	0.999267241036199\\
27	0.998931507267302\\
28	0.998471662934564\\
29	0.99785453556316\\
30	0.997042706041051\\
31	0.995995170040309\\
32	0.994667449210267\\
33	0.993010202766676\\
34	0.990965560160064\\
35	0.988460808885106\\
36	0.985399296825578\\
37	0.981648107502352\\
38	0.977021226696919\\
39	0.971255771498955\\
40	0.963977681586449\\
};
\addlegendentry{Highrise Urban}

\addplot [color=white, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	0.99999\\
13	0.99992\\
14	0.99986\\
15	0.99976\\
16	0.99954\\
17	0.99912\\
18	0.99854\\
19	0.99766\\
20	0.9961\\
21	0.994\\
22	0.99077\\
23	0.98582\\
24	0.9788\\
25	0.96899\\
26	0.95569\\
27	0.93894\\
28	0.91894\\
29	0.89397\\
30	0.86449\\
31	0.82989\\
32	0.79314\\
33	0.75336\\
34	0.71083\\
35	0.66717\\
36	0.62293\\
37	0.58031\\
38	0.53822\\
39	0.49635\\
40	0.45508\\
};
\addlegendentry{\normalsize{Simulations}}

\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	0.99999\\
11	0.99999\\
12	0.99999\\
13	0.99999\\
14	0.99998\\
15	0.99997\\
16	0.99991\\
17	0.99987\\
18	0.99979\\
19	0.99961\\
20	0.99935\\
21	0.99904\\
22	0.99852\\
23	0.99773\\
24	0.9965\\
25	0.99495\\
26	0.99248\\
27	0.98924\\
28	0.98483\\
29	0.97903\\
30	0.97187\\
31	0.96369\\
32	0.95341\\
33	0.94107\\
34	0.92655\\
35	0.90966\\
36	0.89038\\
37	0.86894\\
38	0.84514\\
39	0.81882\\
40	0.79024\\
};


\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	0.99998\\
15	0.99996\\
16	0.99992\\
17	0.99989\\
18	0.99985\\
19	0.99975\\
20	0.99954\\
21	0.99935\\
22	0.99887\\
23	0.99831\\
24	0.99744\\
25	0.99632\\
26	0.99472\\
27	0.99245\\
28	0.98925\\
29	0.9852\\
30	0.97992\\
31	0.97379\\
32	0.96611\\
33	0.9562\\
34	0.94573\\
35	0.93256\\
36	0.91812\\
37	0.90086\\
38	0.88196\\
39	0.85972\\
40	0.83532\\
};


\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	1\\
15	1\\
16	1\\
17	1\\
18	0.99999\\
19	0.99999\\
20	0.99994\\
21	0.99993\\
22	0.99987\\
23	0.99975\\
24	0.99963\\
25	0.99946\\
26	0.99916\\
27	0.99879\\
28	0.99827\\
29	0.99757\\
30	0.99669\\
31	0.99569\\
32	0.9943\\
33	0.99256\\
34	0.99051\\
35	0.98828\\
36	0.98566\\
37	0.98253\\
38	0.97889\\
39	0.9746\\
40	0.96941\\
};


\end{axis}

==> environment_mob.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%


\begin{axis}[%
width=3in,
height=2.3in,
at={(0.1158in,0.081in)},
scale only axis,
xmin=-10,
xmax=35,
xlabel style={font=\color{white!15!black}},
xlabel={SIR Threshold (db)},
ymin=0.65,
ymax=1.05,
ylabel style={font=\color{white!15!black}},
ylabel={succcess probabilty},
axis background/.style={fill=white},
legend style={font=\footnotesize,at={(0.03,0.06)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
-10	0.999999999990738\\
-9	0.999999999981528\\
-8	0.999999999963166\\
-7	0.999999999926563\\
-6	0.999999999853616\\
-5	0.999999999708283\\
-4	0.999999999418844\\
-3	0.999999998842686\\
-2	0.999999997696471\\
-1	0.999999995417898\\
0	0.999999990892578\\
1	0.999999981915778\\
2	0.999999964134998\\
3	0.999999928980801\\
4	0.999999859637713\\
5	0.999999723246649\\
6	0.999999455928343\\
7	0.999998934287223\\
8	0.999997921814\\
9	0.999995969488692\\
10	0.999992234572182\\
11	0.99998515694648\\
12	0.999971894834929\\
13	0.999947368213676\\
14	0.99990268781526\\
15	0.999822663601308\\
16	0.999681997910266\\
17	0.999439691820073\\
18	0.999031162049168\\
19	0.998357657381431\\
20	0.997272937645954\\
21	0.995568057751422\\
22	0.99295658000345\\
23	0.98906424459422\\
24	0.983428114300202\\
25	0.97550963926163\\
26	0.964724363762002\\
27	0.950489609229857\\
28	0.93229049941606\\
29	0.909760785148826\\
30	0.882764604700824\\
31	0.851452468244005\\
32	0.81626194573271\\
33	0.777850560265246\\
34	0.736978800356627\\
35	0.694384668534657\\
36	0.650691801840151\\
37	0.606373064309191\\
38	0.561766223892467\\
39	0.517122063187313\\
40	0.472661889676989\\
};
\addlegendentry{Suburnan}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
-10	0.999999999998498\\
-9	0.999999999997004\\
-8	0.999999999994027\\
-7	0.999999999988092\\
-6	0.999999999976261\\
-5	0.999999999952692\\
-4	0.999999999905752\\
-3	0.99999999981231\\
-2	0.999999999626406\\
-1	0.999999999256827\\
0	0.999999998522781\\
1	0.999999997066545\\
2	0.999999994181802\\
3	0.999999988477647\\
4	0.999999977224082\\
5	0.99999995508476\\
6	0.999999911681536\\
7	0.99999982695695\\
8	0.999999662443081\\
9	0.999999345048847\\
10	0.999998737453618\\
11	0.999997585109726\\
12	0.99999542356953\\
13	0.999991420739141\\
14	0.999984116316539\\
15	0.999971005092795\\
16	0.999947892341675\\
17	0.999907928752363\\
18	0.999840210867661\\
19	0.999727817609894\\
20	0.999545164175324\\
21	0.999254626983007\\
22	0.998802556443625\\
23	0.998115018899891\\
24	0.997093781571443\\
25	0.9956130694058\\
26	0.993517575490588\\
27	0.990622414859799\\
28	0.986716287858479\\
29	0.981569395454303\\
30	0.974946403342627\\
31	0.966621649773141\\
32	0.956390665201985\\
33	0.944071960775231\\
34	0.929497220337476\\
35	0.91249419937389\\
36	0.892870721575034\\
37	0.870407903831561\\
38	0.844867153498164\\
39	0.816011182128231\\
40	0.78363605249935\\
};
\addlegendentry{Urban}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
-10	0.999999999998987\\
-9	0.99999999999798\\
-8	0.999999999995971\\
-7	0.999999999991968\\
-6	0.999999999983988\\
-5	0.999999999968091\\
-4	0.999999999936429\\
-3	0.9999999998734\\
-2	0.999999999748001\\
-1	0.999999999498697\\
0	0.999999999003519\\
1	0.999999998021113\\
2	0.999999996074888\\
3	0.999999992226223\\
4	0.99999998463258\\
5	0.999999969691701\\
6	0.99999994039637\\
7	0.999999883200279\\
8	0.999999772114255\\
9	0.999999557736443\\
10	0.999999147203484\\
11	0.999998368264394\\
12	0.999996906377084\\
13	0.999994197460204\\
14	0.999989250382028\\
15	0.999980362360846\\
16	0.999964677325138\\
17	0.999937522144512\\
18	0.999891439271953\\
19	0.9998148208143\\
20	0.999690051065707\\
21	0.999491105504505\\
22	0.999180654221833\\
23	0.998706859608521\\
24	0.998000168908462\\
25	0.996970412421699\\
26	0.995504490164599\\
27	0.993465081126917\\
28	0.990691235619795\\
29	0.98700198806905\\
30	0.982203416894668\\
31	0.976097560837128\\
32	0.968489391907949\\
33	0.959187686501622\\
34	0.947998166500441\\
35	0.934711397823652\\
36	0.919090978908427\\
37	0.900867852821467\\
38	0.87974457468796\\
39	0.855410649327778\\
40	0.827567768366629\\
};
\addlegendentry{Dense Urban}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
-10	0.999999999999836\\
-9	0.999999999999672\\
-8	0.999999999999347\\
-7	0.999999999998697\\
-6	0.999999999997403\\
-5	0.999999999994825\\
-4	0.999999999989689\\
-3	0.999999999979467\\
-2	0.999999999959129\\
-1	0.999999999918694\\
0	0.999999999838383\\
1	0.999999999679054\\
2	0.999999999363413\\
3	0.999999998739246\\
4	0.999999997507762\\
5	0.999999995084838\\
6	0.999999990334295\\
7	0.99999998105987\\
8	0.999999963048399\\
9	0.999999928292373\\
10	0.999999861742415\\
11	0.999999735490299\\
12	0.999999498589398\\
13	0.999999059711082\\
14	0.999998258464148\\
15	0.999996819461517\\
16	0.999994281125567\\
17	0.999989888797581\\
18	0.999982439028478\\
19	0.999970059517771\\
20	0.999949908902725\\
21	0.999917786075439\\
22	0.999867653084666\\
23	0.99979109624245\\
24	0.999676764913034\\
25	0.999509824834394\\
26	0.999271452583326\\
27	0.998938417828983\\
28	0.998482873532521\\
29	0.997872540355113\\
30	0.997071388123295\\
31	0.996040601221119\\
32	0.994739205654432\\
33	0.993123553606702\\
34	0.99114511837164\\
35	0.988746602010171\\
36	0.985856790376835\\
37	0.982384583225165\\
38	0.978212161351525\\
39	0.973186493646869\\
40	0.967107420315792\\
};
\addlegendentry{Highrise Urban}

\addplot [color=white, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	0.99998\\
13	0.99995\\
14	0.99993\\
15	0.99984\\
16	0.99965\\
17	0.99927\\
18	0.99872\\
19	0.99773\\
20	0.99623\\
21	0.99386\\
22	0.99048\\
23	0.98524\\
24	0.97775\\
25	0.96853\\
26	0.95644\\
27	0.93956\\
28	0.91873\\
29	0.89382\\
30	0.86461\\
31	0.82886\\
32	0.79068\\
33	0.75023\\
34	0.70919\\
35	0.66509\\
36	0.62067\\
37	0.57517\\
38	0.5307\\
39	0.48788\\
40	0.44461\\
};
\addlegendentry{\normalsize{Simulations}}

\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	0.99998\\
13	0.99998\\
14	0.99995\\
15	0.99995\\
16	0.9999\\
17	0.99983\\
18	0.99979\\
19	0.99968\\
20	0.9995\\
21	0.99909\\
22	0.99848\\
23	0.99775\\
24	0.99674\\
25	0.99498\\
26	0.99291\\
27	0.98944\\
28	0.98513\\
29	0.97969\\
30	0.97263\\
31	0.96392\\
32	0.95365\\
33	0.9405\\
34	0.92549\\
35	0.90874\\
36	0.88897\\
37	0.86596\\
38	0.84066\\
39	0.81151\\
40	0.77921\\
};
\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	0.99999\\
15	0.99998\\
16	0.99994\\
17	0.9999\\
18	0.99989\\
19	0.99985\\
20	0.99972\\
21	0.99948\\
22	0.99911\\
23	0.99865\\
24	0.99784\\
25	0.99668\\
26	0.99507\\
27	0.99263\\
28	0.99001\\
29	0.98615\\
30	0.98109\\
31	0.97451\\
32	0.96657\\
33	0.95654\\
34	0.94498\\
35	0.93168\\
36	0.91629\\
37	0.89751\\
38	0.87661\\
39	0.85319\\
40	0.82539\\
};

\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-10	1\\
-9	1\\
-8	1\\
-7	1\\
-6	1\\
-5	1\\
-4	1\\
-3	1\\
-2	1\\
-1	1\\
0	1\\
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	1\\
15	0.99999\\
16	0.99999\\
17	0.99998\\
18	0.99997\\
19	0.99994\\
20	0.99992\\
21	0.99988\\
22	0.99981\\
23	0.99971\\
24	0.99959\\
25	0.99938\\
26	0.99914\\
27	0.9987\\
28	0.99819\\
29	0.99758\\
30	0.99669\\
31	0.99568\\
32	0.99446\\
33	0.99271\\
34	0.99074\\
35	0.98828\\
36	0.98535\\
37	0.9815\\
38	0.97733\\
39	0.97235\\
40	0.96629\\
};
\end{axis}

==> environment_sta.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%


\begin{axis}[%
width=3in,
height=2.3in,
at={(0.758in,0.481in)},
scale only axis,
xmin=-20,
xmax=20,
xlabel={SINR  (dB)},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Success probability},
axis background/.style={fill=white},
legend style={font=\footnotesize,at={(0.6,0.62)}, anchor=south west, legend cell align=left, align=left, draw=white!10!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
-40	0.992120774039563\\
-39	0.990092473093017\\
-38	0.987602063449647\\
-37	0.984895285154533\\
-36	0.981534664712672\\
-35	0.977351872187002\\
-34	0.972631772593022\\
-33	0.96678001634779\\
-32	0.959356105273149\\
-31	0.950337410519553\\
-30	0.93971486628775\\
-29	0.928994139550821\\
-28	0.91508370478108\\
-27	0.899612942757221\\
-26	0.881944034977831\\
-25	0.862154358987689\\
-24	0.840148247451449\\
-23	0.816809188095504\\
-22	0.7920934461513\\
-21	0.764243855381369\\
-20	0.735093269998999\\
-19	0.704103840436859\\
-18	0.673566848604145\\
-17	0.640397011181617\\
-16	0.606410418083543\\
-15	0.573053850187457\\
-14	0.539219196794293\\
-13	0.507489595572973\\
-12	0.477845890291687\\
-11	0.447186525794507\\
-10	0.420628847951851\\
-9	0.396110339321829\\
-8	0.372928011137456\\
-7	0.351367652641979\\
-6	0.332344513236282\\
-5	0.316147595722608\\
-4	0.301914533873266\\
-3	0.28981729482451\\
-2	0.278722731148611\\
-1	0.26975942812426\\
0	0.261501027405228\\
1	0.255979542775714\\
2	0.251516937020434\\
3	0.24676939238473\\
4	0.243072506923035\\
5	0.24010480196527\\
6	0.237427403277919\\
7	0.235711051218335\\
8	0.233508519905546\\
9	0.232478850890869\\
10	0.231678422011324\\
11	0.230247725978762\\
12	0.229191055695468\\
13	0.227559260215789\\
14	0.225385204587938\\
15	0.222849325472656\\
16	0.220791195766797\\
17	0.217911203775934\\
18	0.215200601544698\\
19	0.211061484275825\\
20	0.205701102225035\\
21	0.201290462375848\\
22	0.195031579257381\\
23	0.188300427453156\\
24	0.18097578938208\\
25	0.173586691762223\\
26	0.164582528940279\\
27	0.155392514733684\\
28	0.146434189018989\\
29	0.138085308449816\\
30	0.127746048008154\\
31	0.116549083731889\\
32	0.108262256923765\\
33	0.0995351330419039\\
34	0.0890619991201341\\
35	0.07921583456159\\
36	0.0702811888617554\\
37	0.0657845021168783\\
38	0.0596302720195469\\
39	0.0515839477389421\\
40	0.0448025233445417\\
};
\addlegendentry{Suburnan}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
-40	0.993991951562138\\
-39	0.992100118199013\\
-38	0.990273702185004\\
-37	0.988148374478064\\
-36	0.985313161857023\\
-35	0.982314260280401\\
-34	0.978765050852367\\
-33	0.974083855933323\\
-32	0.969205984094923\\
-31	0.96246312956239\\
-30	0.955310089204411\\
-29	0.946115570041631\\
-28	0.935352871176105\\
-27	0.922281568055097\\
-26	0.908558750834093\\
-25	0.890854643764383\\
-24	0.871159299777874\\
-23	0.85071400759321\\
-22	0.826966574410238\\
-21	0.801480220131234\\
-20	0.773252156864097\\
-19	0.742560078829242\\
-18	0.710686596794863\\
-17	0.67579236099581\\
-16	0.638846687308835\\
-15	0.601607260972157\\
-14	0.564019184747042\\
-13	0.524899658902269\\
-12	0.485151660140362\\
-11	0.445451469557325\\
-10	0.409589697603666\\
-9	0.373893929863857\\
-8	0.342437263611747\\
-7	0.311447395616885\\
-6	0.28270861621242\\
-5	0.258059507148334\\
-4	0.237673476410653\\
-3	0.21731182838966\\
-2	0.201339393879024\\
-1	0.184111511289499\\
0	0.169016042244627\\
1	0.156121965109624\\
2	0.144200207277847\\
3	0.131591956495894\\
4	0.121183599241649\\
5	0.113473350871751\\
6	0.106215737695333\\
7	0.100012903457746\\
8	0.0950724811062113\\
9	0.0903121782420133\\
10	0.0861527894459111\\
11	0.0827493751607143\\
12	0.0796440248896429\\
13	0.0769908335976727\\
14	0.0742727820784268\\
15	0.0718986102481303\\
16	0.0694761235829671\\
17	0.0676928872198524\\
18	0.0656265157086978\\
19	0.0635109933560524\\
20	0.0619717984392203\\
21	0.0598920350620397\\
22	0.0577588251174896\\
23	0.056013216902886\\
24	0.0540059909339815\\
25	0.0514669673841362\\
26	0.0490421803536994\\
27	0.0469007167604665\\
28	0.0444587151603856\\
29	0.0417453853854044\\
30	0.0387192759977234\\
31	0.0359143369411311\\
32	0.0340451321589073\\
33	0.0322818500416\\
34	0.0304178202108489\\
35	0.0279599636350521\\
36	0.0267137950552568\\
37	0.0252123391196695\\
38	0.023229871682621\\
39	0.0225766394599545\\
40	0.0215991230348106\\
};
\addlegendentry{Urban}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
-40	0.995193002719611\\
-39	0.993981767043418\\
-38	0.992365974444355\\
-37	0.990023818271903\\
-36	0.987810155619477\\
-35	0.985069480500878\\
-34	0.98178761737875\\
-33	0.977627750259391\\
-32	0.972974004399979\\
-31	0.966694330175946\\
-30	0.959577359628857\\
-29	0.951239934742694\\
-28	0.941368220601673\\
-27	0.929390831974993\\
-26	0.915540840872673\\
-25	0.900435849794037\\
-24	0.88248073207303\\
-23	0.862713128110255\\
-22	0.841360360207164\\
-21	0.81673998070972\\
-20	0.790203971137916\\
-19	0.761492360680677\\
-18	0.728781354889234\\
-17	0.69346932584749\\
-16	0.657295492998015\\
-15	0.620666149012206\\
-14	0.581590789394688\\
-13	0.541182428978013\\
-12	0.502088756773627\\
-11	0.462503539224355\\
-10	0.425254594006696\\
-9	0.388489897191568\\
-8	0.353115223171261\\
-7	0.322078007494964\\
-6	0.292484307508988\\
-5	0.265670114215782\\
-4	0.241305759279393\\
-3	0.220064677887685\\
-2	0.19967233682092\\
-1	0.182414952445866\\
0	0.166846368487593\\
1	0.15478165456822\\
2	0.141597397299457\\
3	0.128905158946782\\
4	0.118730116570576\\
5	0.109434002014825\\
6	0.100646293908153\\
7	0.0934225060485202\\
8	0.0872138166829413\\
9	0.0817519775258301\\
10	0.0771862670002317\\
11	0.073086347505604\\
12	0.0691168631025288\\
13	0.0652223345583667\\
14	0.0618775389915323\\
15	0.0589598476160603\\
16	0.0563623453551505\\
17	0.0546838348293241\\
18	0.052256666551477\\
19	0.0499308454089984\\
20	0.0478965444231971\\
21	0.0458597376285105\\
22	0.0438778406050207\\
23	0.0418101066997183\\
24	0.0397570630952647\\
25	0.0380743875605749\\
26	0.035674180310081\\
27	0.0331241320208559\\
28	0.0306803431226324\\
29	0.0281146943142788\\
30	0.0259723088200755\\
31	0.023976260921645\\
32	0.0224618184288973\\
33	0.0211183420438434\\
34	0.0196458865478552\\
35	0.0175058274026117\\
36	0.0159266366040729\\
37	0.0154218657669297\\
38	0.0138990845571066\\
39	0.0132930844704701\\
40	0.0131535425047939\\
};
\addlegendentry{Dense Urban}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
-40	0.998357272538784\\
-39	0.998163700384711\\
-38	0.997706111953504\\
-37	0.997298523340845\\
-36	0.996673521840078\\
-35	0.996040902870267\\
-34	0.994989483053874\\
-33	0.993604564867825\\
-32	0.991808023506355\\
-31	0.989538870252984\\
-30	0.987228387476506\\
-29	0.984564689855927\\
-28	0.98198807801713\\
-27	0.97773480191957\\
-26	0.973042458724965\\
-25	0.966882900446968\\
-24	0.96062386879132\\
-23	0.953574591163594\\
-22	0.943671000728497\\
-21	0.93206333501965\\
-20	0.919600312624824\\
-19	0.903676781241307\\
-18	0.886405704482613\\
-17	0.866484502815163\\
-16	0.841197275433887\\
-15	0.813828492110235\\
-14	0.78179490031295\\
-13	0.748099276898924\\
-12	0.709057122020918\\
-11	0.665752461208336\\
-10	0.620367868522263\\
-9	0.572819774020419\\
-8	0.525998984986288\\
-7	0.478501427969552\\
-6	0.432340067011314\\
-5	0.388794447874624\\
-4	0.35002146282701\\
-3	0.31342950945798\\
-2	0.278562590383457\\
-1	0.248199313304996\\
0	0.221520263529752\\
1	0.198595832712436\\
2	0.176744602638757\\
3	0.161488320192635\\
4	0.144560612173507\\
5	0.128766182548789\\
6	0.118002193340351\\
7	0.108113643631078\\
8	0.0932098178361388\\
9	0.0815658984669992\\
10	0.074058105635414\\
11	0.0667258767986906\\
12	0.0601949951891211\\
13	0.0545672777168948\\
14	0.0491207911352059\\
15	0.0441164833286388\\
16	0.0397579966200712\\
17	0.0360193977768097\\
18	0.0325237157914789\\
19	0.0291593709404498\\
20	0.0267396040336401\\
21	0.0241831592581459\\
22	0.0222258588624371\\
23	0.0206367980350499\\
24	0.0185977020135921\\
25	0.0162676141825816\\
26	0.0147965642011081\\
27	0.0135426765021322\\
28	0.0120359609107723\\
29	0.0109073621159932\\
30	0.00959408586184153\\
31	0.00847860785148758\\
32	0.00742614980604899\\
33	0.00648103484747805\\
34	0.00581871262358737\\
35	0.00494955318064358\\
36	0.00427362122554695\\
37	0.00384184947567846\\
38	0.0036579047533262\\
39	0.0035930395560096\\
40	0.0025799423642533\\
};
\addlegendentry{High-rise Urban}

\addplot [color=white, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-40	0.99192\\
-38	0.98744\\
-36	0.98116\\
-34	0.97178\\
-32	0.95784\\
-30	0.93826\\
-28	0.91228\\
-26	0.87812\\
-24	0.8356\\
-22	0.78628\\
-20	0.72908\\
-18	0.66716\\
-16	0.59982\\
-14	0.53318\\
-12	0.47092\\
-10	0.4141\\
-8	0.36706\\
-6	0.3275\\
-4	0.29746\\
-2	0.27492\\
0	0.25872\\
2	0.24772\\
4	0.2402\\
6	0.23498\\
8	0.23118\\
10	0.22902\\
12	0.22596\\
14	0.22212\\
16	0.21718\\
18	0.2105\\
20	0.20066\\
22	0.18938\\
24	0.17488\\
26	0.15826\\
28	0.1398\\
30	0.12044\\
32	0.10212\\
34	0.08394\\
36	0.06712\\
38	0.05266\\
40	0.04058\\
};
\addlegendentry{\normalsize{Simulations}}

\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-40	0.9937\\
-38	0.9902\\
-36	0.98516\\
-34	0.97852\\
-32	0.96796\\
-30	0.95388\\
-28	0.9338\\
-26	0.90712\\
-24	0.86896\\
-22	0.82296\\
-20	0.76726\\
-18	0.7035\\
-16	0.63252\\
-14	0.55826\\
-12	0.48092\\
-10	0.40606\\
-8	0.34052\\
-6	0.2814\\
-4	0.23418\\
-2	0.19436\\
0	0.16286\\
2	0.13922\\
4	0.1211\\
6	0.10702\\
8	0.0957\\
10	0.08678\\
12	0.08014\\
14	0.07476\\
16	0.06982\\
18	0.06586\\
20	0.06218\\
22	0.05788\\
24	0.05368\\
26	0.04864\\
28	0.04384\\
30	0.0385\\
32	0.03394\\
34	0.02952\\
36	0.02508\\
38	0.02162\\
40	0.01826\\
};
\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-40	0.99522\\
-38	0.99234\\
-36	0.98768\\
-34	0.98156\\
-32	0.97248\\
-30	0.95894\\
-28	0.94066\\
-26	0.9145\\
-24	0.88118\\
-22	0.8394\\
-20	0.78786\\
-18	0.72634\\
-16	0.6543\\
-14	0.57898\\
-12	0.50078\\
-10	0.4243\\
-8	0.35298\\
-6	0.29166\\
-4	0.23768\\
-2	0.1964\\
0	0.163\\
2	0.1364\\
4	0.11518\\
6	0.09858\\
8	0.08636\\
10	0.07652\\
12	0.0686\\
14	0.06132\\
16	0.05598\\
18	0.05198\\
20	0.04764\\
22	0.04344\\
24	0.0394\\
26	0.03518\\
28	0.03078\\
30	0.02648\\
32	0.02232\\
34	0.0188\\
36	0.0159\\
38	0.01346\\
40	0.01158\\
};
\addplot [color=black, draw=none, mark=x, thin, mark size=2pt, mark options={ black}]
  table[row sep=crcr]{%
-40	0.99844\\
-38	0.99772\\
-36	0.9968\\
-34	0.99494\\
-32	0.99158\\
-30	0.98692\\
-28	0.98148\\
-26	0.97282\\
-24	0.95992\\
-22	0.94244\\
-20	0.91802\\
-18	0.88432\\
-16	0.83908\\
-14	0.77918\\
-12	0.7062\\
-10	0.6178\\
-8	0.5234\\
-6	0.4301\\
-4	0.34654\\
-2	0.27552\\
0	0.21998\\
2	0.17516\\
4	0.13986\\
6	0.11212\\
8	0.08886\\
10	0.07204\\
12	0.05864\\
14	0.0479\\
16	0.0386\\
18	0.03158\\
20	0.02602\\
22	0.02174\\
24	0.01796\\
26	0.01444\\
28	0.01182\\
30	0.00936\\
32	0.00756\\
34	0.00586\\
36	0.0043\\
38	0.00344\\
40	0.00252\\
};


\end{axis}
